Safe Dependency Atoms and Possibility Operators in Team Semantics

I consider the question of which dependencies are safe for a Team Semantics-based logic FO(D), in the sense that they do not increase its expressive power over sentences when added to it. I show that some dependencies, like totality, non-constancy and non-emptiness, are safe for all logics FO(D), and that other dependencies, like constancy, are not safe for FO(D) for some choices of D despite being strongly first order. I furthermore show that the possibility operator, which holds in a team if and only if its argument holds in some nonempty subteam, can be added to any logic FO(D) without increasing its expressive power over sentences.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{A. Orlandini, M. Zimmermann (Eds.): 9th Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF'18)\\
EPTCS 277, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.277.5}{10.4204/EPTCS.277.5}}

